ConceptCarve: Dynamic Realization of Evidence

Finding evidence for human opinion and behavior at scale is a challenging task, often requiring an understanding of sophisticated thought patterns among vast online communities found on social media. For example, studying how gun ownership is related to the perception of Freedom, requires a retrieval system that can operate at scale over social media posts, while dealing with two key challenges: (1) identifying abstract concept instances, (2) which can be instantiated differently across different communities. To address these, we introduce ConceptCarve, an evidence retrieval framework that utilizes traditional retrievers and LLMs to dynamically characterize the search space during retrieval. Our experiments show that ConceptCarve surpasses traditional retrieval systems in finding evidence within a social media community. It also produces an interpretable representation of the evidence for that community, which we use to qualitatively analyze complex thought patterns that manifest differently across the communities.

==> latex/sections/background.tex <==
\section{Background and Related Work} IR aims to retrieve relevant documents from large collections based on user queries.

\textbf{Inferential Gap:} The \textbf{lexical gap}, or \emph{vocabulary mismatch}, arises when query and document vocabularies differ. We differentiate between: (1) A \textbf{shallow gap}, resolved by simple rewording to increase overlap, and (2) An \textbf{inferential gap}, requiring complex reasoning and nontrivial inferences (Figure~\ref{fig:gap-example}). Our dataset highlights this inferential gap, which existing datasets do not specifically address. 

Several approaches have been proposed to address the lexical gap problem using LLMs. Generally, the retriever component in Retrieval Augmented Generation (RAG) seeks to improve factuality and memory of a generative agent \cite{gao2024retrievalaugmentedgenerationlargelanguage}. Thus, many works attempt to improve retrieval for an information need \cite{asai2023self, jiang2023activeretrievalaugmentedgeneration, ma-etal-2023-query, pham-etal-2024-whos}, emphasizing generation using top results, not attempting to realize a query within a corpus. 

Several works use LLM embeddings or use LLMs to train smaller retrievers \cite{wang-etal-2024-improving-text, dai2022promptagatorfewshotdenseretrieval, 10.1145/3626772.3657951, yoon-etal-2024-matryoshka, yoon-etal-2024-search}. These works run orthogonal to our own, as our method is agnostic to the retriever, leaving room for any improvements from LLM-based retrievers. Other works use LLMs not as the backbone retriever, but as a tool to reformulate the query \cite{wang2023query2doc, jagerman2023query}. While very cheap, these methods do not interact with the retrieved results, relying solely on an LLM's prediction of relevant results (query expansion).

\textbf{Domain Sensitivity:} We identify the challenge of adapting a domain-sensitive query to the search domain, termed \textbf{ad-hoc domain adaptation} to emphasize that the retriever must adapt to the data \emph{at every query}. Particularly, when there exists an inferential gap, but the inference required to resolve it is highly dependent on the search domain. Figure~\ref{fig:gap-example} demonstrates how the realization of a trend can be extremely sensitive to the dataset being searched.

Various works tackle domain sensitivity via either adapting the retrieval model to the data, or utilizing pseudo-relevance feedback (PRF) \cite{10.1145/383952.383972, 10.1145/1645953.1646259} during search. Parametric methods \cite{saadfalcon2023udapdr, Wang_2022, jiang-etal-2023-boot, zhou-etal-2023-enhancing-generative, wang-etal-2023-effective} adapt the retriever to a specific domain via training. Domain information is also added in other ways, as in \citet{n2022injecting, 10.1162/tacl_a_00530}. Other PRF methods use document embeddings to improve a second retrieval/reranking \cite{Zheng_2020, Wang_2021, gao2022precisezeroshotdenseretrieval, shen2023largelanguagemodelsstrong}, or use an LLM to expand the query with some interactions \cite{jia-etal-2024-mill, weller-etal-2024-generative, chen-etal-2024-analyze, lei-etal-2024-corpus}.

However, these methods tend to: (1) rely on parametric learning; (2) omit recursive refinement of search components; (3) use small initial document sets, limiting their ability to characterize the corpus; or (4) lack interpretability because they are not concept-based, making it difficult to understand the motivation behind the model's results.

Concurrently with our work, \citet{weller2024promptrieverinstructiontrainedretrieversprompted} introduce \emph{Promptriever}, a retrieval model designed to be prompted like a language model. Their method also targets the inferential gap, but does so by parametrically modifying the model through training. In contrast, our approach is concept-based and interpretable, without requiring changes to the retriever itself.

A few works have created abstract, interpretable explanations of text corpora \cite{Lam_2024, NEURIPS2023_7e810b2c, wang-etal-2023-goal}, while others do this by characterizing frames, perspectives, and stances in a social science setting \cite{roy-goldwasser-2023-tale, roy-goldwasser-2020-weakly, reuver-etal-2024-topic, ziems-yang-2021-protect-serve, pujari-goldwasser-2021-understanding, pacheco-etal-2023-interactive}; however, these methods do not use retrievers and are limited to downsampling or smaller datasets when using LLMs.

Most similar to our work is \citet{hoyle-etal-2023-natural}, who represent implicit text explicitly for opinion mining, but must downsample the corpus for LLM use. Likewise, \citet{ravfogel2024descriptionbasedtextsimilarity} search text via abstract descriptions, though they use an LLM for data generation to \emph{train} an encoder. Both methods do not address the issue of domain-sensitivity, which is at the heart of this paper.



==> latex/sections/concept_carve.tex <==
\section{Concept Carve}
Here, we define terms used in the \textsc{ConceptCarve} framework, followed by the framework itself.

\subsection{Definitions}

\textbf{Intent:} An \emph{intent} is the user's goal in retrieval, expressed as text. In our setting, the intent is to ``find evidence'' for a trend in human behavior, but it could be any goal. For example, ``Find evidence that teens are using vaping products in public schools.'' Alternatively, it could be ``get ideas,'' like ``Give me ideas on how to decorate my room using minimalism.'' Figure~\ref{fig:bank-example} shows a complex intent.

\noindent
\textbf{Grounding:} A \emph{grounding} is a single string which can be used as a query with a standard retriever. Figure~\ref{fig:bank-example} (right) depicts several examples.

\noindent
\textbf{Concept:} A \emph{concept} is an abstract idea, represented by a set of groundings (as seen in Figure~\ref{fig:bank-example}). For convenience, concepts can be named; though only groundings are ever used. A concept acts as a bridge: concrete enough for retrieval (using groundings), yet compact enough for LLM reasoning. 

\noindent
\textbf{Concept Tree:} A \emph{concept tree} is a tree of weighted concepts. Positively-weighted concepts are \emph{promoted} and negatively-weighted concepts are \emph{demoted}. By carefully adding promoted and demoted concepts, the tree can carve out a complex intent (Figure~\ref{fig:bank-example}). For example, it allows for promoting a broad idea while downplaying certain aspects, in addition to allowing for iterative refinement by interacting with the data.

\subsection{Framework}

\captionsetup[figure]{labelfont={small}, textfont={small}}
\begin{figure*}[h]
    \centering
    \includegraphics[width=\linewidth]{diagrams/ConceptCarveDiagram.png}
    \caption{\small\textsc{ConceptCarve}: a concept tree is recursively constructed in steps $1\ldots t$ by alternating between Characterizer (generates new concepts from intermediate docs) and Retriever (retrieves docs using intermediate trees). Output tree represents the realization of the input trend within the input community and can be used for evidence retrieval or analyzed directly.}
    \label{fig:framework-diagram}
\end{figure*}

The framework consists of the main module, Characterizer, and its submodule, Retriever. The Characterizer interactively grows a concept tree, repeatedly using the Retriever to get intermediate results. Figure~\ref{fig:framework-diagram} gives an overview of the framework.

\subsubsection{Retriever}

The \emph{Retriever} utilizes an off-the-shelf retrieval engine, $E$ and a concept tree $T$ (which may be partially built) to either rerank or retrieve from a set of documents $D$. In the Characterizer section, we explain how the Retriever's operations are used repeatedly to grow a tree. While most retrieval systems use a query to calculate a document's relevance score, the Retriever uses a concept tree. $T$ can embody some (potentially) complicated idea, and so we use its concepts' groundings and the off-the-shelf retriever $E$ to calculate the score.

To compute the relevance score for a document $d$ to the tree $T$, we use all of its concepts' groundings: Let $C$ be the set of concepts in $T$, and $G_c$ be the set of groundings for concept $c$. Let $w(c)$ denote the weight of concept $c$ in $T$. Finally, let $\rho_E(g, d)$ denote the relevance score assigned by $E$ to $d$ with grounding $g$. Then $T$'s assigned relevance score to $d$ is given by equation~\ref{eq:rep-relevance}.
\vspace{-0.5em}
\begin{equation}
\rho_T(d) = \sum_{c \in C} \sum_{g \in G_c} w(c) \times \rho_E(g, d)
\label{eq:rep-relevance}
\end{equation}
\vspace{-1em}

We simply use the off-the-shelf engine to find the relevance of the document for each grounding of each concept, and add them up, weighting them via the respective concept's weight. We do this for every document in a small set $D_q$ to perform reranking, as shown in equation~\ref{eq:rep-rerank}. We can also do this scoring for every document in the whole dataset $D$, and rank all documents to perform end-to-end retrieval. When this is the case, the retriever returns a set of top $k$ documents according to the scoring function, as shown in equation~\ref{eq:rep-end-to-end-retrieve}. \vspace{-0.35em}
\begin{equation}
\operatorname{rerank}(T, D_q) = \{ (d, \rho_T(d)) \mid d \in D_q \}
\label{eq:rep-rerank}
\end{equation}
\vspace{-1em}
\begin{equation}
\fontsize{10.375pt}{11pt}\selectfont
\operatorname{retrieve}(T, D, k) = \text{top-}k \{ (d, \rho_T(d)) \mid d \in D \}
\label{eq:rep-end-to-end-retrieve}
\end{equation}


Two things should be noted: (1) demoted concept weights are negative, and hence relevance to demoted concepts reduces the relevance of a document, and (2) the concept tree structure of $T$ is not taken into account when calculating a document's relevance to $T$. That is, the simplicity of the relevance scoring relies heavily on the high quality of the concepts, groundings, and weights of $T$.

\subsubsection{Characterizer}
The \emph{Characterizer} grows a concept tree for some intent over some dataset. At a high level, it does this by judiciously using an LLM to inspect retrieved documents, forming concepts, and reasoning over which concepts should be promoted and which should be demoted. Importantly, the Characterizer is the only component which requires reasoning, and therefore is the only component which requires an LLM. The input to the Characterizer is an intent $i$, a dataset $D$, and a $k$ indicating the size of each intermediate retrieval. Its output is a carved concept tree $T$ representing $i$ as it manifests in $D$.

The algorithm begins with a root concept (single-node tree), which, when retrieved, should provide a starting point for the Characterizer. In our implementation, we create the root by making a concept whose grounding is just $i$, though any initialization is possible (as in Figure~\ref{fig:bank-example}).

To grow out a concept's children, the Characterizer performs three high-level operations: (1) \textbf{ancestor path retrieval:} retrieve using an intermediate concept tree, (2) \textbf{envision/explore:} cluster the retrieved documents, creating groups of documents that support/refute the intent, and (3) \textbf{concept induction:} extract properties from each group and use them to generate groundings for new concepts (the new children). To grow the whole tree, these operations are performed recursively, starting at the root. We now explain each operation in detail.

\begin{table*}[!ht]
    \small
    \centering
    \begin{tabular}{l|ccc|ccc|ccc}
        \hline
        \textbf{Reranking System} & \multicolumn{3}{c|}{@10} & \multicolumn{3}{c|}{@100} & \multicolumn{3}{c}{@500} \\
        \cline{2-10}
        & P & R & MAP & P & R & MAP & P & R & MAP \\
        \hline
        BM25 & 13.20 & 0.70 & 0.30 & 12.90 & 6.10 & 1.10 & 12.70 & 27.50 & 3.80 \\
        ColBERT & 26.10 & 1.30 & 0.60 & 21.00 & 9.20 & 2.50 & 16.70 & 34.80 & 7.10 \\
        ANCE & 23.70 & 1.30 & 0.60 & 18.70 & 8.70 & 2.20 & 16.00 & 33.40 & 6.50 \\
        RepLLaMA & 14.11 & 0.53 & 0.23 & 13.42 & 5.04 & 0.94 & 15.05 & 29.84 & 4.49 \\
        Query2Doc + ColBERT & 37.28 & 2.20 & 1.33 & 26.57 & 13.42 & 4.82 & 19.59 & 42.43 & 11.37 \\
        MultiQuery + ColBERT & 25.20 & 1.33 & 0.71 & 19.89 & 9.49 & 2.60 & 16.42 & 35.49 & 7.08 \\
        \textsc{Envision Only} & 38.00 & 2.10 & 1.20 & 28.20 & 14.40 & 5.10 & 20.70 & 46.00 & 12.50 \\
        \textsc{ConceptCarve} (depth 1) & \underline{40.11} & \underline{2.39} & \underline{1.46} & \underline{29.83} & \underline{15.75} & \underline{5.80} & \underline{21.44} & \underline{48.86} & \underline{13.81} \\
        \textsc{ConceptCarve} (depth 2) & \textbf{41.56} & \textbf{2.40} & \textbf{1.49} & \textbf{30.70} & \textbf{16.38} & \textbf{6.10} & \textbf{21.78} & \textbf{49.71} & \textbf{14.33} \\
        \hline
    \end{tabular}
    \caption{Performance on the DIR task. The best is \textbf{bolded}, and the second best \underline{underlined}.}
    \label{tab:dataset-informed-results}
\end{table*}


\textbf{Ancestor Path Retrieval:}
Given a concept $c$, we wish to inspect which documents it contributes to the whole tree's retrieval. Since $c$ may depend on other concepts in the tree for its meaning, we isolate its entire ancestor path—the subtree containing all nodes from the root to $c$. Then, using the ancestor path as a concept tree in itself, we apply the Retriever's $\operatorname{retrieve}$ operation to get the top $k$ documents from the dataset $D$ that are most relevant to the path. We call this set $D_{ret}$.

\textbf{Envision/Explore:}
The \textbf{explore} operation aims to inspect $D_{ret}$ and find useful ideas within it, while the \textbf{envision} operation aims to inspect $D_{ret}$ and expand the search space by introducing new ideas. First, we cluster $D_{ret}$ using BERTopic \cite{grootendorst2022bertopic}. In both operations, the top $m$ clusters (each with $n$ centroid documents) are presented to an LLM. In \textbf{explore}, the LLM identifies clusters that support or refute the intent. For \textbf{envision}, an LLM generates centroids that the LLM deems \emph{should} support the intent but are missing from the clusters. The result of both operations is a set of clusters that either support or refute the intent.

\textbf{Concept Induction:}
The final step is to convert these clusters into concepts, a process we call \textbf{concept induction}. To create a concept, we need a set of groundings. For supporting clusters, we provide an LLM with the cluster's centroids and the intent $i$, asking it to generate properties explaining why the documents support $i$. The same process is done for refuting clusters, explaining why they do not support $i$. The LLM then synthesizes these properties into artificial documents, which serve as the groundings for the new concept. For convenience, the LLM also names the concepts, though the names are not used in retrieval.

\textbf{Weighting:}
The weighting scheme chosen gives lesser weights to children than parents, ensures equality among siblings, and normalizes the weights. Intuitively, this means that a subconcept can only partially counteract its superconcept. Details are in Appendix~\ref{app:weighting}.

\textbf{Reranking:} Finally, since we wish to use the final concept tree $T$ for reranking a set of documents $D_q$, we can simply call $\operatorname{rerank}(T, D_q)$.


==> latex/sections/conclusion.tex <==
\section{Conclusion}
We introduced \textsc{ConceptCarve}, a retrieval framework that combines traditional retrievers with LLM-guided concept construction to adapt to specific communities. It addresses two major challenges in evidence retrieval: the inferential gap and ad-hoc domain adaptation. Unlike LLM-based query expansion or embedding methods, \textsc{ConceptCarve} iteratively builds a concept tree, leading to stronger performance and greater interpretability.

Our experiments show that \textsc{ConceptCarve} outperforms both traditional and LLM-augmented baselines, despite using no training or fine-tuning. Its effectiveness across a large, diverse dataset highlights its potential for retrieving and analyzing how communities express complex opinions and behaviors.

Future work includes refining concept weighting schemes and exploring how trends evolve over time or align with real-world events. We hope this framework inspires further research at the intersection of retrieval, reasoning, and human-centered analysis.

==> latex/sections/discussion_and_analysis.tex <==
\section{Discussion and Analysis}
We detail E2E retrieval analysis, a qualitative analysis of the trees, and the costs of \textsc{ConceptCarve}.

\textbf{E2E Retrieval:}
Demoting concepts in pilot experiments didn't improve reranking. This may be because the reranking set was made from ColBERT's top $2000$ results, which were already aligned with the trend, lacking noise to be removed. To test this, we performed E2E retrieval using concept trees with, and without demoted concepts. In reranking, the document set is fixed, but here we measure how many `evidence' examples are retrieved, using only P@k as a metric, labeling on the fly. Since such labeling is expensive, we used 24 trend-community pairs (48K posts), and analysis was limited to testing demoted concepts.

\begin{table}
    \small
    \setlength{\tabcolsep}{3pt}
    \centering
  \begin{tabular}{lcccccc}
    \hline
    \textbf{Retriever} & P@5 & P@10 & P@50 & P@100 & P@500 & P@1K \\
    \hline
    ColBERT & 27.8 & 25.4 & 22.5 & 20.9 & 16.7 & 14.9 \\
    \textsc{CC} ($+$) & 30.8 & \textbf{34.2} & 29.8 & 25.8 & 19.8 & 17.9\\
    \textsc{CC} ($+-$) & \textbf{34.2} & 32.9 & \textbf{30.7} & \textbf{26.9} & \textbf{20.4} & \textbf{18.0}\\
    \hline
    \end{tabular}
    \caption{Performance on the end-to-end retrieval task, with ($+-$) and without ($+$) demoted concepts.}
    \label{tab:retrieval-ablation}
\end{table}

\textbf{E2E Results:} Table~\ref{tab:retrieval-ablation} shows the E2E results, ablating the demoted concepts. The results show that including demoted concepts slightly improves the precision of the retrieved results. We hypothesize that the improvement is small since the retrieval process is very sensitive to the weighting difference in promoted and demoted concepts. Despite this, the results support our hypothesis that demoted concepts reduce the relevance score of irrelevant posts when retrieving from the full dataset.

\textbf{Concept Tree Qualitative Analysis:}
We show that concept-carved trees provide interpretable realizations of trends across communities. To compare communities, we construct concept trees for the same trend within opposing communities (e.g., rural vs. urban). During construction, each concept is grounded via concept induction, where an LLM identifies key properties that make evidence ``supporting.'' These are then analyzed to extract polarity—differences in evidence priority between communities (e.g., ``mentions/does not mention mental health''). These polarities are visualized to highlight how communities realize evidence differently.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{diagrams/spider3.png}
    \caption{Trend: ``Increase in frustration with family members who seem to prioritize personal ambitions over traditional family values.''}
    \label{fig:spider3}
\end{figure}

In Figure~\ref{fig:spider3}, we compare the concept trees for the \emph{rural} and \emph{urban} communities. Using the trees' properties, an LLM identifies polarities and scores their usefulness in identifying evidence for the trend in each community. The spider plot shows that, for the urban community, social media effects strongly indicate evidence. In contrast, rural evidence emphasizes conflict over traditional family expectations, while urban evidence focuses on conflict related to a family's image. Plots for other trends/communities are in Appendix~\ref{app:more-qual-analysis}. This analysis reveals both \emph{how} \textsc{ConceptCarve} retrieves evidence, and qualitatively demonstrates that the trees represent each community's realization.

\textbf{Cost Analysis:}  
\textsc{ConceptCarve}'s cost includes characterization and retrieval. The Characterizer's dominant cost is the number of LLM calls, measured asymptotically in input tokens. With $B$ as the branching factor, $m$ as the clusters shown during envision/explore, and $n$ as the centroid documents per cluster, the Characterizer's cost is $O(B^2n + Bmn)$. In our implementation, this equates to $\sim$20,000 tokens per tree, \textbf{independent of dataset size} and number of reranked/retrieved documents $k$. Thus, while our method incurs a higher initial query cost, it scales efficiently to massive datasets. Retrieval cost, measured in retriever calls, is $O(C \times \gamma)$, where $\gamma$ is the number of groundings per concept and $C$ is the total number of concepts. Appendix~\ref{app:cost-analysis} provides detailed derivations and examines accuracy trade-offs.



==> latex/sections/experiments.tex <==
\section{DIR Evaluation}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{diagrams/map_plot2.png}
    \caption{MAP@k on DIR task.}
    \label{fig:map-plot}
\end{figure}

This section details Dataset-informed Reranking (DIR), performed on the constructed dataset.

\textsc{ConceptCarve} allows various tree configurations. We can limit the promoted (PBF), demoted (DBF), and envisioned branching factors (EBF), as well as tree depth. After pilot tests, we set PBF, EBF, and DBF to 5, with a maximum depth of 2, since concept weights diminished beyond that. For reranking, we only used promoted concept nodes, as the benefit of demoted concepts in reranking was not seen (see end-to-end retrieval as to why).

Our baselines were as follows. \textbf{BM25:} \cite{inproceedings} a lexical retrieval model. \textbf{ANCE:} \cite{xiong2020approximate} a dense, exact search bi-encoder model. \textbf{ColBERT:} \cite{Khattab_2020} a late interaction retriever. \textbf{Query2Doc + ColBERT:} \cite{wang2023query2doc} an LLM expands the query into a hypothetical document, then reranks with ColBERT. \textbf{MultiQuery + ColBERT:} \cite{langchain_multiqueryretriever} an LLM rewrites the query three times, then reranks using ColBERT on all three. \textbf{RepLLaMA:} \cite{ma2023finetuningllamamultistagetext} a dense retriever which uses LLaMA-2-7B as its backbone. \textbf{\textsc{EnvisionOnly}:} a version of \textsc{ConceptCarve} where concepts come only from the \textbf{envision} operation (what the LLM sees as missing from intermediate results). Reproducibility details in Appendix~\ref{app:reproducibility}.

\textbf{DIR Results:}
Table~\ref{tab:dataset-informed-results} and Figure~\ref{fig:map-plot} show that \textsc{ConceptCarve} outperforms all baseline reranking models. Models using an LLM, including the \textsc{EnvisionOnly} and Query2Doc, significantly outperform dense and lexical models, highlighting the LLM's ability to address the inferential gap. Both \textsc{ConceptCarve} models, especially at depth 2, surpass \textsc{EnvisionOnly} and Query2Doc, demonstrating the benefit of interacting with the data during tree construction. This shows the utility of the \textbf{explore} operation and the ability of the dataset to test ad hoc domain adaptation. Finally, depth 2 slightly outperforms depth 1, indicating that exploring more concepts improves trend realization.

\textbf{Generality and Dataset Diversity:}
While our evaluation uses a single data source (Reddit), the dataset spans over 3,000 subreddits within a wide range of domains, including politics, religion, hobbies, employment, education, and online culture. This results in over 165 million posts for tree construction and 360,000 for reranking. The diversity in topic, style, and community norms offers a broad and challenging testbed for evidence realization. Notably, \textsc{ConceptCarve} operates without any training or tuning, using only an off-the-shelf ColBERT retriever and an LLM, yet performs very well across this diverse data. We argue that this setting provides strong evidence of the framework’s capacity to generalize across communities and topics in the task of realizing evidence of human behavior and opinion.

==> latex/sections/introduction.tex <==
\section{Introduction}
Human behavior and opinion are notoriously complex, particularly when mining textual resources in order to understand them \citep{kang-etal-2023-values, paulissen-wendt-2023-lauri, He_Wang_Zhao_Yang_2024}. If done well, a system that accurately quantifies human opinion at scale could supplement expensive polls and potentially reduce reliance on them. Likewise, it could demonstrate patterns in preferences like dietary habits~\cite{pilavr2021healthy,hashimoto2024meat} or vaccine hesitancy~\cite{zhang2023moral,qorib2023covid}. These patterns, which we refer to as \emph{trends}, capture the collective tendencies, attitudes, beliefs, or behaviors within a specific community or context. However, due to the complexity of human thought and expression, finding and quantifying supporting textual evidence of these trends is difficult, as it requires an understanding of what such evidence would look like in text (i.e. the \emph{realization} of the evidence).
%
\begin{figure}[!t]
    \centering
    \resizebox{\columnwidth}{!}{
    \def\vdist{2.7} % Adjust this value to change the spacing between boxes
    \def\yone{3}    % Starting y-coordinate for the first set of boxes
    \def\ytwo{\yone - \vdist}
    \def\ythree{\ytwo - \vdist}
    \def\yfour{\ythree - \vdist}
    \begin{tikzpicture}[
        query/.style={rectangle, draw=yellow!50, fill=yellow!20, thick, minimum height=1.5cm, text width=4.2cm, align=center, font=\Large},
        document/.style={rectangle, draw=green!50, fill=green!20, thick, minimum height=1.5cm, text width=5.9cm, align=center, font=\Large},
        redbox/.style={rectangle, draw=red!50, fill=red!20, thick, minimum height=2cm, text width=2.95cm, align=center, font=\Large},
        bluebox/.style={rectangle, draw=blue!50, fill=blue!20, thick, minimum height=2cm, text width=2.55cm, align=center, font=\Large},
        arrow/.style={->, thick, shorten >=1pt, >=stealth}
    ]
    
    % Labels for each pair (rotated, spaced, and wrapped)
    \node[rotate=90, text=black, text width=2cm, align=center] at (-3.15, \yone) {\Large \textbf{No Lexical Gap}};
    \node[rotate=90, text=black, text width=2.75cm, align=center] at (-3.15, \ytwo) {\Large \textbf{Shallow Gap}};
    \node[rotate=90, text=black, text width=2.75cm, align=center] at (-3.15, \ythree) {\Large \textbf{Inferential Gap}};
    \node[rotate=90, text=black, text width=2.75cm, align=center] at (-3.15, \yfour) {\Large \textbf{Domain Sensitive Query}};
    
    % Query 1
    \node[query] (query1) at (0, \yone) {What is rappelling?};
    \node[document] (doc1) at (6, \yone) {Rappelling is the process of coming down from a mountain...};
    \draw[arrow] (query1) -- (doc1);
    
    % Query 2
    \node[query] (query2) at (0, \ytwo) {Health benefits of antioxidant-rich foods};
    \node[document] (doc2) at (6, \ytwo) {Eating items rich in compounds that fight free radicals can enhance wellness by protecting cells...};
    \draw[arrow] (query2) -- (doc2);
    
    % Query 3
    \node[query] (query3) at (0, \ythree) {Expression of having freedom};
    \node[document] (doc3) at (6, \ythree) {I emptied my car's tank today. Turning 16 could not have been better...};
    \draw[arrow] (query3) -- (doc3);
    
    % Query 4 - New pair with a split document box
    \node[query] (query4) at (0, \yfour) {Expression of having freedom};
    
    % Red box aligned with left edge of other document boxes
    \node[redbox, anchor=west] (doc4a) at (2.9, \yfour) {Go Second Amendment! \#GunOwner};
    
    % Blue box aligned with right edge of other document boxes
    \node[bluebox, anchor=east] (doc4b) at (9, \yfour) {My body, my choice! \#RoeVWade};
    
    % Add labels under the red and blue boxes
    \node at ([yshift=-0.25cm]doc4a.south) {\Large (conservative)};
    \node at ([yshift=-0.25cm]doc4b.south) {\Large  (liberal)};
    
    % Arrow from query to red box
    \draw[arrow] (query4) -- (doc4a);
    
    % Titles or labels
    \node at (0, \yone + 1.25) {\large \textbf{Query}};
    \node at (6, \yone + 1.25) {\large \textbf{Relevant Document}};
    
    \end{tikzpicture}
    }
    \caption{Example of no lexical gap, shallow gap, inferential gap, and domain sensitivity in a retrieval task.}
    \label{fig:gap-example}
\end{figure}

Realizing evidence requires inferring how people express a given trend in text (e.g., when seeking evidence of people having ``freedom'', what kinds of things would they say?). Additionally, understanding the search space itself is crucial for this inference (the evidence for people having ``freedom'', is likely to be different across liberal and conservative communities (Figure~\ref{fig:gap-example})). This motivates the need for a method that can \emph{adapt to the search space}.

Large Language Models (LLMs) have demonstrated remarkable reasoning capabilities in recent years \citep{brown2020languagemodelsfewshotlearners, chen2021evaluatinglargelanguagemodels, rae2022scalinglanguagemodelsmethods}. Since human analysis of large corpora is infeasible, a strong alternative is an LLM that analyzes every single textual document and infers its evidential value. However, doing so would be extremely expensive and time consuming (for example, even a few hundred thousand posts on Reddit would cost thousands of dollars to annotate using OpenAI's GPT-4o model).

In contrast, the Information Retrieval (IR) community has developed light and fast retrieval models capable of searching enormous corpora with impressive accuracy \citep{10.1145/3637870, 10.1145/3486250, zhu2024largelanguagemodelsinformation}. Despite this, these models continue to struggle in cases when the lexical overlap between a query and its relevant documents is low (known as the \emph{lexical gap}) (Figure~\ref{fig:gap-example}) \cite{zhu2024largelanguagemodelsinformation}. While attempts to address the lexical gap have shown promise, they overlook \emph{domain sensitivity}, a problem that occurs when the meaning of the query is sensitive to the search domain (e.g. ``freedom'' for liberals and conservatives), and can only be addressed by adapting to the domain.

This paper aims to bridge the gap between the inefficiency of LLMs and the limited inferential capabilities of IR models, while ensuring adaptability to specific domains. We leverage the strong reasoning capabilities of LLMs to carve out a realization of a trend's evidence within a particular community. We are motivated to use a concept-based method due to its \textbf{interpretability} and \textbf{scalability}. Crucially, our method does not require LLM inference on the whole corpus, operating within a fixed budget of LLM tokens which \textbf{does not depend on the size of the corpus}, making it scalable to large datasets. Our proposed method incrementally allows an LLM to interact with fast retrievers in order to discover the boundaries of the trend being searched \emph{as it is realized in a community} (Figure~\ref{fig:framework-diagram}).

Via this process, our method is able to fit the realization to the community and define a nuanced representation of it. We call this process \textsc{\textbf{ConceptCarve}}, as it is akin to starting with a crude slab of material and carving out a detailed representation of a real-life object. After Concept Carving a trend in human thought patterns, the resulting representation can be used to (1) quickly retrieve evidence from a large dataset (for quantification), and (2) interpret how evidence is realized within a specific community (qualitative analysis). 

Moral Foundations Theory (MFT) is a framework that categorizes the underlying values driving human moral reasoning, and has been thoroughly used by social scientists for two decades \cite{fd3cbcce-5e3f-39a6-b275-9a1d627a0c23, Haidt2007WhenMO, graham2013moral}. These foundations (such as care/harm, fairness/cheating, and loyalty/betrayal) have been shown to manifest differently across groups of people \cite{Khan02042016}. Thus, to reveal the necessity of adaptation to data, we construct a dataset of Reddit posts, partitioned by several communities (e.g. liberal and conservative), and use our approach to find evidence of trends in these moral foundations among various groups. 

We frame `finding evidence' as a reranking task, wherein \textsc{ConceptCarve} supersedes all baselines, achieving a 120.46\% relative improvement in MAP@500 over a dense reranking model, and a 26.03\% relative improvement in MAP@500 over an LLM keyword expansion technique.

To qualitatively analyze the resulting carved representations, we show that they can be used to automatedly detect features that separate two communities for some trend. For example, using our approach, we looked at the trend in \emph{``family members not recognizing desire for freedom''}, among \textbf{liberals} and \textbf{conservatives} and note that evidence of this trend among liberals is realized as discussion of \emph{`personal identity and space'}, while among conservatives, the evidence is realized as \emph{`parental control'} and \emph{`family recognition'}. These analyses demonstrate that \textsc{ConceptCarve} offers significant potential as a tool for both quantifying opinions and capturing their realization across communities. Our contributions can be summarized as: 
\vspace{-2.0em}
\begin{enumerate}
    \setlength{\itemsep}{0pt}
    \setlength{\parskip}{0pt}
    \item Introduce \textsc{ConceptCarve}, a method for dynamically realizing evidence of a trend within a community.
    \item Introduce a dataset which tests a model's ability to deal with (1) inferential gap, and (2) domain sensitivity on the evidence-finding task.\footnote{We release the dataset at \url{https://huggingface.co/datasets/ecaplan/conceptcarve}}
    \item Demonstrate that \textsc{ConceptCarve} outperforms baselines on the dataset.
    \item Use \textsc{ConceptCarve}'s carved representations to analyze how evidence of moral foundations is realized in various communities.
\end{enumerate}





==> latex/sections/limitations_ethics.tex <==
\section*{Limitations} The Reddit data used in our experiments does not represent the full spectrum of online discussions, limiting the generalizability of our results to other platforms or domains. Additionally, LLMs were used extensively for data annotation, which introduces potential biases inherent in these models. While we manually validated some LLM labels, the overall quality and fairness of the labels may still be affected by the limitations of the LLMs themselves.

\section*{Ethics Statement}
LLMs were used extensively in this work, and we acknowledge their potential for bias due to the nature of their training data. All products of LLMs, including complex frameworks, should be critically evaluated and not taken at face value when real-world consequences are involved. To mitigate risks, we applied human oversight whenever possible. All datasets used were either publicly available or collected with proper consent, ensuring data privacy. We are committed to ethical AI use, fairness, and transparency throughout this project.

==> latex/sections/problem_formulation.tex <==
\section{Problem Formulation}
In this section, we describe the formal definitions of the tasks, then outline our dataset's construction.

\subsection{Task Definitions}
An \textbf{end-to-end} (E2E) retrieval task considers a set of documents $D$ and a set of queries $Q$. The dataset comes with labeled relevance scores, which can be formulated as a function $\rho: D \times Q \rightarrow \mathbb{R}$, where $\mathbb{R}$ is the set of real numbers, though most datasets either work in binary relevance $\{0,1\}$ or other discrete relevance judgments. The retrieval engine's task is to approximate $\rho$ with its own relevance function, which we denote $\hat{\rho}(d, q)$ for all pairs $(d, q)$. This means that for any pair $(d,q)$, we want to minimize the distance $| \rho(d,q) - \hat{\rho}(d,q) |$.

The \textbf{reranking} task is very similar, except that for each query $q$, a subset of $D$ of size $k$ is selected by the dataset's creators beforehand to be reranked, which we denote $D_q$. Normally, $D_q$ is generated by the top $k$ results of a lightweight, fast retrieval engine on $D$ using $q$. The task is to approximate $\rho$ with a relevance function $\rho_{rerank}: D \times Q \rightarrow \mathbb{R}$, such that $\rho_{rerank}(d, q)$ is similar to $\rho(d,q)$ for all $q$ and $d \in D_q$. In traditional reranking methods, the reranker uses only $D_q$ to rerank documents. However, we believe that even when reranking $D_q$, there is important information garnered from $D$ itself. Subtle observations about the dataset may help inform reranking decisions in a small subset.

We define our task: \textbf{dataset-informed reranking} (DIR), where the task of producing $\rho_{rerank}$ remains the same, but the model has full access to $D$ while reranking $D_q$. To span multiple domains, in our setting we break $D$ into specialized sub-datasets $D_1, D_2, ..., D_n$ and for each, generate a reranking subset $D_{i, q}$ for every query $q \in Q$.

\subsection{Dataset Design}
To fully demonstrate the utility of our framework, we desired the following two features: (1) that the queries require complex inference to relate them to documents (inferential gap) and (2) that the same query manifests differently across different datasets, such as `freedom' in liberal vs. conservative sub-datasets (ad-hoc domain adaptation).

\textbf{Reddit:} We chose Reddit to be our source of social media data because (1) it was diverse in topics and user demographics, (2) it was available via the Cornell ConvoKit project \cite{convokit}, and (3) its segmentation into subreddits enables a natural way of making online communities into sub-datasets. ConvoKit allows access up to 10/2018.

\textbf{Community Definitions:} To obtain sub-datasets, we first defined three pairs of contrasting \uline{communities}: liberal/conservative (political ideology), urban/rural (population density), and religious/secular (spirituality). These were chosen for Reddit availability, distinctiveness, and relevance to social science, for a total of \textbf{six communities}.

\textbf{Community Sub-datasets:} After defining the communities, we collected the top $100,000$ subreddits by size from ConvoKit. We concatenated the subreddit's name with its description, and used an sBERT model's cosine similarity to retrieve the top $10,000$ most similar subreddits for each community. We only kept subreddits which the LLM labeled as `predominantly used by the target community'. We then randomly sampled posts. Table~\ref{tab:community_posts_subreddits} shows the number of posts and subreddits in each community, and Appendix~\ref{app:dataset-details} provides more details, including each community's top subreddits and community overlap. Finally, we had a large dataset $D_c$ for each community $c$.

\begin{table}[ht]
    \small
  \centering
  \begin{tabular}{l c c}
    \hline
    \textbf{Community} & \textbf{\# of Posts (in M)} & \textbf{\# of Subreddits} \\
    \hline
    Conservative          & 44.6  & 268 \\
    Liberal               & 28.2  & 976 \\
    Rural                 & 23.9  & 485 \\
    Urban                 & 19.9  & 1221 \\
    Religious             & 15.4  & 299 \\
    Secular               & 33.6  & 142 \\
    \hline
  \end{tabular}
  \caption{Community, number of posts in the dataset, and number of subreddits sampled to generate it.}
  \label{tab:community_posts_subreddits}
\end{table}

\begin{figure*}[ht!]
    \centering
    % Left side: Original Tree Diagram (now on the left)
    \begin{subfigure}[t]{0.65\textwidth}
    \centering
    \hspace{-3cm}
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[
        remember picture,
        node_style/.style={
            rectangle, draw, line width=1.5pt, minimum width=1cm, minimum height=1cm, align=center, font=\Large\ttfamily,
            double copy shadow={shadow xshift=5pt, shadow yshift=-5pt, opacity=.4},
        },
        edge_style/.style={draw, line width=2pt},
        sibling distance=2.5cm,
        level 1/.style={sibling distance=4cm, level distance=1.5cm, edge from parent/.style=edge_style},
        level 2/.style={sibling distance=3.5cm, every child/.style={xshift=0cm}, level distance=1.75cm, edge from parent/.style=edge_style},
        level 3/.style={sibling distance=4cm, level distance=1.75cm, edge from parent/.style=edge_style},
        font=\small,
    ]

    \tikzset{
        red_color/.style={fill={rgb,255:red,255;green,150;blue,150}, text=black},
        green_color/.style={fill={rgb,255:red,170;green,255;blue,170}, text=black},
        blue_color/.style={fill={rgb,255:red,145;green,235;blue,255}, text=black},
        background/.style={rectangle, fill=gray!20, inner sep=0.4cm, rounded corners=5mm},
    }

    \node[node_style, blue_color] (bank) {Bank (+0.5)}
        child {node[node_style, red_color] (cash) {Cash (-0.1)}}
        child {node[node_style, red_color] (money) {Money (-0.2)}}
        child {node[node_style, green_color] (river) {River (+0.23)}
            child {node[node_style, red_color] (fastcurrents) {Fast Currents\\(-0.17)}}
            child {node[node_style, red_color] (polluted) {Polluted\\(-0.12)}}
            child {node[node_style, red_color] (unsafe) {Unsafe\\(-0.12)}}
            child {node[node_style, green_color] (stones) {Stones\\(+0.07)}
                child {node[node_style, red_color] (small) {Small (-0.08)}}
                child {node[node_style, red_color] (rough) {Rough (-0.06)}}
                child {node[node_style, green_color] (big) {Big (+0.01)}}
                child {node[node_style, green_color] (smooth) {Smooth (+0.02)}}}
            child {node[node_style, green_color] (shallow) {Shallow\\(+0.08)}}
            child {node[node_style, green_color] (clearwater) {Clear Water\\(+0.09)}}};

    % Background rectangle with coordinates
    \begin{scope}[on background layer]
        \node[background, fit=(clearwater), name=smallbox, inner sep=15pt] {};
    \end{scope}
    % Coordinates for corners of the small gray box
    \coordinate (smallboxtr) at (smallbox.north east);
    \coordinate (smallboxbr) at (smallbox.south east);

    \end{tikzpicture}
    }
    \end{subfigure}
    % \hspace{1cm}
    % \vspace{-0.5cm}
    % \hspace{1cm}
    % Right side: Zoomed-in Clear Water with additional nodes (now on the right)
    \begin{subfigure}[t]{0.15\textwidth}
        \begin{tikzpicture}[
            remember picture,
            node_style/.style={
                rectangle, draw, minimum width=1.5cm, minimum height=0.5cm, align=center, font=\scriptsize\ttfamily,
            },
            light_node_style/.style={
                rectangle, draw, minimum width=0.5cm, minimum height=0.75cm, text width=2.5cm, align=center, font=\scriptsize, inner sep=1pt
            },
        ]

        \def\top{-2}
        \def\bot{1}
        \def\left{0}
        \def\right{4}
        
        % Gray box background with coordinates for corners
        \coordinate (bigboxbl) at (\left, \bot);
        \coordinate (bigboxtl) at (\left, \top);
        \coordinate (bigboxbr) at (\right, \bot);
        \coordinate (bigboxtr) at (\right, \top);
        \begin{scope}
            \fill[gray!20, rounded corners=0.5cm] (bigboxbl) rectangle (bigboxtr);
        \end{scope}

        \clip (current bounding box.south west) rectangle (current bounding box.north east);

        % Define colors
        \definecolor{green_color}{RGB}{170, 255, 170}
        \colorlet{light_green_color}{green_color!40!white}

        % Node styles
        \tikzset{
            green_color_node/.style={fill=green_color, text=black},
            light_green_color_node/.style={fill=light_green_color, text=black},
        }

        % Node positions
        \node[node_style, green_color_node] (clearwater) at ($(1.4, 2.5) + (\left, \top)$) {Clear Water (+0.09)};

        % Offsets
        \def\dx{0.25}
        \def\dy{-0.715}
        \def\dxone{0.6}
        \def\dyone{-0.575}

        % Additional nodes
        \node[light_node_style, light_green_color_node] (node1) at ($(clearwater) + (\dxone,\dyone)$) {``You can see everything---it's safe.''};

        \node[light_node_style, light_green_color_node] (node2) at ($(node1) + (\dx,\dy)$) {``This water’s super clean.''};

        \node[light_node_style, light_green_color_node] (node3) at ($(node2) + (\dx,\dy)$) {``Nothing scary is hiding under there.''};

        \node[light_node_style, light_green_color_node] (node2) at ($(node2)$) {``This water’s super clean.''};

        \node[light_node_style, light_green_color_node] (node1) at ($(node1)$) {``You can see everything---it's safe.''};

        \node[node_style, green_color_node] (clearwater) at ($(clearwater)$) {Clear Water (+0.09)};

        \end{tikzpicture}
    \end{subfigure}

    % Draw lines connecting the corners
    \begin{tikzpicture}[remember picture, overlay]
        \draw[-, ultra thick, gray!20] ($(bigboxtl) + (0.15cm,0.15cm)$) -- (2.3, 1.15);
        \draw[-, ultra thick, gray!20] ($(bigboxbl) + (0.18cm,-0.15cm)$) -- (2.3, 2.05);
    \end{tikzpicture}

    \begin{tikzpicture}[remember picture, overlay]
    \node at (current page.center) [yshift=12cm] { % Adjust yshift as needed
        \parbox[b]{5.75cm}{ % Adjust width as needed
            \centering
            \small
            \textbf{Intent:} ``give descriptions of the river bank of a river that has big, smooth stones, and is safe for swimming''
        }
    };
\end{tikzpicture}

    
    \caption{\small(Left): Concept tree: promoted (green) and demoted (red) concepts. Note that this tree sets the root to the ambiguous `Bank'; our Characterizer would have used the full intent. (Right): Concept of ``Clear Water'', displayed with its set of groundings.}
    \label{fig:bank-example}
\end{figure*}



\textbf{Trends:} Independently of the communities and our framework, we systematically generated complex, domain-sensitive trends to be our queries. To ensure they were \textbf{domain-sensitive}, we chose each query to be a trend based on a moral foundation, since we know that moral foundations manifest differently across communities \cite{Khan02042016}. First, we created a list of 6 base trends, each of the form ``Increase in belief that people feel X'', where ``X'' is the positive end of the moral foundation (caring, fairness, loyalty etc.) 

Since we desired an \textbf{inferential gap}, we did not want simple trends whose evidence could be determined by discussion topic. Thus, to induce the queries to be more complex, we defined several \uline{complexity dimensions}: time (how opinions change over time), relationships (influence of social connections), evidence (whether opinions are based on personal or objective sources), emotions (impact on emotional states), agency (who is acting or affected), and scope (whether changes occur at an individual or societal level). Then, we asked an LLM to qualify each trend with 5 distinct combinations of 2-3 complexity dimensions. The result was 30 complex, domain-sensitive trends, which we used as our set of queries $Q$. The full list of trends can be found in Appendix~\ref{app:dataset-details}.


\textbf{Reranking Set:} 
To construct the reranking subset $D_{c,q}$ for each query $q$ and community $c$, a mix of relevant and non-relevant posts was needed. Since the trends are so specific, finding relevant posts was nontrivial. We used the ColBERT retriever \cite{Khattab_2020} to form a reranking set for each pair $c, q$. For each query, $k=2000$ posts were retrieved from $D_c$ to form the subset $D_{c,q}$. ColBERT was chosen for its speed and semantic retrieval capabilities, as simpler lexical searches likely wouldn't yield sufficient evidence. The choice of retrieval engine does not affect the final task since the goal is to rerank the results.

\textbf{Labeling} To label the relevance of each post in $D_{c,q}$, we had an LLM label each $d \in D_{c,q}$ by asking if $d$ is evidence of $q$ (prompt in Appendix~\ref{app:prompts}, no mention of community $c$). This 0/1 label was used for evaluating reranking. The final dataset consists of: (1) 30 independent, complex, domain-sensitive trends, (2) 6 community sub-datasets $D_{rural}, D_{urban},$... (3) 180 sets of 2000 posts, and each post labeled as evidence/not evidence (one set for each trend/community pair).

\textbf{Human Validation}
Over 12 hours of human annotations show 68\% agreement with LLM labels and 70\% inter-annotator agreement (see Appendix~\ref{app:dataset-details}). While our goal is to align with LLM judgments rather than humans', these results minimally validate the LLM's judgments for this task.





==> old/old_results.tex <==
\begin{table*}[!ht]
    \small
  \centering
  \begin{tabular}{lcccccc}
    \hline
    \textbf{Reranking System} & P@5 & P@10 & P@50 & P@100 & P@500 & P@1000 \\
    \hline
    BM25 & 0.1260 & 0.1320 & 0.1330 & 0.1290 & 0.1270 & 0.0700 \\
    ColBERT & 0.2740 & 0.2610 & 0.2290 & 0.2100 & 0.1670 & 0.1500 \\
    ANCE (dense) & 0.2500 & 0.2370 & 0.2020 & 0.1870 & 0.1600 & 0.1470 \\
    Query2Doc 0-shot & 0.3967 & 0.3728 & 0.2963 & 0.2657 & 0.1959 & 0.1656 \\
    Query2Doc few-shot & 0.3667 & 0.3456 & 0.2856 & 0.2614 & 0.1921 & 0.1624 \\
    Query2Doc q+d 0-shot & 0.3944 & 0.3561 & 0.2826 & 0.2588 & 0.1919 & 0.1622 \\
    Query2Doc q+d few-shot & 0.3578 & 0.3478 & 0.2872 & 0.2613 & 0.1924 & 0.1618 \\
    \textsc{Envision Only} & 0.4110 & 0.3800 & 0.3100 & 0.2820 & 0.2070 & 0.1720 \\
    \textsc{ConceptCarve} (depth 1) & 0.4356 & 0.4011 & 0.3278 & 0.2983 & 0.2144 & 0.1757 \\
    \textsc{ConceptCarve} (depth 2) & \textbf{0.4456} & \textbf{0.4156} & \textbf{0.3382} & \textbf{0.3070} & \textbf{0.2178} & \textbf{0.1775} \\
    \hline
    \textbf{Reranking System} & R@5 & R@10 & R@50 & R@100 & R@500 & R@1000 \\
    \hline
    BM25 & 0.0040 & 0.0070 & 0.0320 & 0.0610 & 0.2750 & 0.5180\\
    ColBERT & 0.0070 & 0.0130 & 0.0530 & 0.0920 & 0.3480 & 0.5980 \\
    ANCE (dense) & 0.0070 & 0.0130 & 0.0500 & 0.0870 & 0.3340 & 0.5910 \\
    Query2Doc 0-shot & 0.0124 & 0.0220 & 0.0796 & 0.1342 & 0.4243 & 0.6764 \\
    Query2Doc few-shot & 0.0107 & 0.0198 & 0.0751 & 0.1311 & 0.4191 & 0.6656 \\
    Query2Doc q+d 0-shot & 0.0122 & 0.0215 & 0.0728 & 0.1276 & 0.4165 & 0.6610 \\
    Query2Doc q+d few-shot & 0.0103 & 0.0203 & 0.0751 & 0.1294 & 0.4198 & 0.6628 \\
    \textsc{Envision Only} & 0.0120 & 0.0210 & 0.0820 & 0.1440 & 0.4600 & 0.7110 \\
    \textsc{ConceptCarve} (depth 1) & 0.0130 & 0.0239 & 0.0902 & 0.1575 & 0.4886 & 0.7330 \\
    \textsc{ConceptCarve} (depth 2) & \textbf{0.0134} & \textbf{0.0240} & \textbf{0.0948} & \textbf{0.1638} & \textbf{0.4971} & \textbf{0.7389} \\
    \hline
    \textbf{Reranking System} & MAP@5 & MAP@10 & MAP@50 & MAP@100 & MAP@500 & MAP@1000\\
    \hline
    BM25 & 0.0020 & 0.0030 & 0.0070 & 0.0110 & 0.0380 & 0.0700\\
    ColBERT & 0.0040 & 0.0060 & 0.0170 & 0.0250 & 0.0710 & 0.1110 \\
    ANCE (dense) & 0.0040 & 0.0060 & 0.0150 & 0.0220 & 0.0650 & 0.1040 \\
    Query2Doc 0-shot & 0.0088 & 0.0133 & 0.0329 & 0.0482 & 0.1137 & 0.1603 \\
    Query2Doc few-shot & 0.0074 & 0.0115 & 0.0296 & 0.0451 & 0.1085 & 0.1532 \\
    Query2Doc q+d 0-shot & 0.0082 & 0.0122 & 0.0291 & 0.0438 & 0.1070 & 0.1514 \\
    Query2Doc q+d few-shot & 0.0069 & 0.0112 & 0.0293 & 0.0447 & 0.1080 & 0.1521 \\
    \textsc{Envision Only} & 0.0080 & 0.0120 & 0.0330 & 0.0510 & 0.1250 & 0.1740 \\
    \textsc{ConceptCarve} (depth 1) & 0.0094 & 0.0146 & 0.0382 & 0.0580 & 0.1381 & 0.1886 \\
    \textsc{ConceptCarve} (depth 2) & \textbf{0.0096} & \textbf{0.0149} & \textbf{0.0399} & \textbf{0.0610} & \textbf{0.1433} & \textbf{0.1944} \\
    \hline
  \end{tabular}
  \caption{Performance on the dataset-informed reranking task.}
  \label{tab:dataset-informed-results}
\end{table*}

\begin{table*}
    \small
    \centering
  \begin{tabular}{lcccccc}
    \hline
    \textbf{Retrieval System} & P@5 & P@10 & P@50 & P@100 & P@500 & P@1000 \\
    \hline
    \textsc{ConceptCarve} (+) & 0.308 & \textbf{0.342} & 0.298 & 0.258 & 0.198 & 0.179\\
    \textsc{ConceptCarve} (+, -) & \textbf{0.342} & 0.329 & \textbf{0.307} & \textbf{0.269} & \textbf{0.204} & \textbf{0.180}\\
    \hline
    \textbf{Retrieval System} & MAP@5 & MAP@10 & MAP@50 & MAP@100 & MAP@500 & MAP@1000\\
    \hline
    \textsc{ConceptCarve} (+) & \textbf{0.666} & 0.516 & \textbf{0.409} & 0.359 & 0.282 & 0.238\\
    \textsc{ConceptCarve} (+, -) & 0.650 & \textbf{0.526} & 0.394 & \textbf{0.365} & \textbf{0.291} & \textbf{0.242}\\
    \hline
    \end{tabular}
    \caption{Performance on the end-to-end retrieval task, with and without the demoted concepts.}
    \label{tab:retrieval-ablation}
\end{table*}

==> old/old_tree_diagram.tex <==
\begin{figure*}[t]
    \centering
    % Left side: Zoomed-in Clear Water with additional nodes
    \begin{subfigure}[t]{0.3\textwidth}
        \begin{tikzpicture}[
            remember picture,
            node_style/.style={
                ellipse, draw, minimum width=1.5cm, minimum height=0.75cm, align=center, font=\scriptsize,
            },
            light_node_style/.style={
                rectangle, draw, minimum width=1cm, minimum height=0.75cm, align=center, font=\tiny, inner sep=4pt, rounded corners=4mm
            },
        ]

        % Gray box background with coordinates for corners
        \coordinate (bigboxbl) at (-6, -2.5);
        \coordinate (bigboxtl) at (-6, 2.5);
        \coordinate (bigboxbr) at (0, -2.5);
        \coordinate (bigboxtr) at (0, 2.5);
        \fill[gray!20, rounded corners=0.5cm] (bigboxbl) rectangle (bigboxtr);
        % Define colors
        \definecolor{green_color}{RGB}{8,148,28}
        \colorlet{light_green_color}{green_color!60!white}

        % Node styles
        \tikzset{
            green_color_node/.style={fill=green_color, text=white},
            light_green_color_node/.style={fill=light_green_color, text=white},
        }

        % Node positions
        \node[node_style, green_color_node] (clearwater) at (-5, 1.5) {Clear\\Water\\(+0.09)};

        % Offsets
        \def\dx{1.2}
        \def\dy{-1.1}
        \def\dxone{1.4}
        \def\dyone{-1.1}

        % Additional nodes
        \node[light_node_style, light_green_color_node] (node1) at ($(clearwater) + (\dxone,\dyone)$) {``When the water’s\\clear, you know you’re\\good to go.''};

        \node[light_node_style, light_green_color_node] (node2) at ($(node1) + (\dx,\dy)$) {``Safe as it gets—\\this river’s clean\\and see-through.''};

        \node[light_node_style, light_green_color_node] (node3) at ($(node2) + (\dx,\dy)$) {``Clear water means\\no surprises, just\\smooth sailing.''};

        \end{tikzpicture}
        \label{fig:\thefigure a}  % Reference will be like Figure Xa
        % \label{fig:zoomed-clearwater}
    \end{subfigure}
    \hfill
    % Right side: Original Tree Diagram
    \begin{subfigure}[t]{0.6\textwidth}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tikzpicture}[
        remember picture,
        node_style/.style={
            ellipse, draw, minimum width=0.5cm, minimum height=0.5cm, align=center, font=\small,
            double copy shadow={shadow xshift=2pt, shadow yshift=-3pt, opacity=.4},
        },
        edge_style/.style={draw, -{Stealth[]}, thick},
        sibling distance=2.5cm,
        level 1/.style={sibling distance=5cm, level distance=1.75cm},
        level 2/.style={sibling distance=2.75cm, every child/.style={xshift=0cm}, level distance=2.5cm},
        level 3/.style={sibling distance=2.75cm, level distance=2cm},
        font=\small,
    ]

    \tikzset{
        red_color/.style={fill={rgb,255:red,255;green,0;blue,0}, text=white},
        green_color/.style={fill={rgb,255:red,8;green,148;blue,28}, text=white},
        blue_color/.style={fill={rgb,255:red,24;green,112;blue,209}, text=white},
        background/.style={rectangle, fill=gray!20, inner sep=0.4cm, rounded corners=5mm},
    }

    \node[node_style, blue_color] (bank) {Bank\\(+0.5)}
        child {node[node_style, green_color] (river) {River\\(+0.23)}
            child {node[node_style, green_color] (clearwater) {Clear\\Water\\(+0.09)}}
            child {node[node_style, green_color] (shallow) {Shallow\\(+0.08)}}
            child {node[node_style, green_color] (stones) {Stones\\(+0.07)}
                child {node[node_style, green_color] (smooth) {Smooth\\(+0.02)}}
                child {node[node_style, green_color] (big) {Big\\(+0.01)}}
                child {node[node_style, red_color] (rough) {Rough\\(-0.06)}}
                child {node[node_style, red_color] (small) {Small\\(-0.08)}}}
            child {node[node_style, red_color] (unsafe) {Unsafe\\(-0.12)}}
            child {node[node_style, red_color] (polluted) {Polluted\\(-0.12)}}
            child {node[node_style, red_color] (fastcurrents) {Fast\\Currents\\(-0.17)}}}
        child {node[node_style, red_color] (money) {Money\\(-0.2)}}
        child {node[node_style, red_color] (cash) {Cash\\(-0.1)}};

    % Background rectangle with coordinates
    \begin{scope}[on background layer]
        \node[background, fit=(clearwater), name=smallbox] {};
    \end{scope}
    % Coordinates for corners of the small gray box
    \coordinate (smallboxtl) at (smallbox.north west);
    \coordinate (smallboxbl) at (smallbox.south west);

    \end{tikzpicture}
    }
    

    
    \label{fig:\thefigure b}  % Reference will be like Figure Xb
\end{subfigure}

    % Draw lines connecting the corners
    \begin{tikzpicture}[remember picture, overlay]
        \draw[-, ultra thick, gray!20] ($(bigboxtr) + (-0.15cm,-0.2cm)$) -- ($(smallboxtl) + (0cm,-2.05cm)$);
        \draw[-, ultra thick, gray!20] ($(bigboxbr) + (-0.25cm,0.1cm)$) -- ($(smallboxbl) + (0cm,-0.5cm)$);
    \end{tikzpicture}
    \caption{(Left): Concept of ``Clear Water'', displayed with its groundings. (Right): Concept tree of the intent ``river bank of a river that has big, smooth stones, and is safe for swimming''. Promoted concepts are shown in green, while demoted concepts are shown in red. Concept weights are displayed as part of each node. Each node also has a set of \emph{groundings}, as shown for the `Clear Water' node.}
    % \captionsetup[subfigure]{labelformat=custom}
    % \renewcommand{\thesubfigure}{\thefigure\alph{subfigure}} % Labels as Xa, Xb, etc.
    
    % \caption*{\textbf{(a)} Subfigure 1, \textbf{(b)} Subfigure 2}
    \label{fig:bank-example}
\end{figure*}


